First-principles study of the energetics and the local chemical ordering of tungsten-based alloys

Tungsten (W) is considered a leading candidate for structural and functional materials in future fusion energy devices. The most attractive properties of tungsten for magnetic and inertial fusion energy reactors are its high melting point, high thermal conductivity, low sputtering yield, and low long-term disposal radioactive footprint. However, tungsten also presents a very low fracture toughness, primarily associated with inter-granular failure and bulk plasticity, limiting its applications. In recent years, several families of tungsten-based alloys have been explored to overcome the aforementioned limitations of pure tungsten. These might include tungsten-based high-entropy alloys (W-HEAs) and the so-called tungsten-based "smart alloys". In this work, we present a computational approach that uses first-principles DFT electronic structure calculations to understand the effect of the chemical environment on tungsten-based alloys. In particular, we compared the Special Quasi-random Structure (SQS) and the DFT-coupled Monte Carlo (MC-DFT) methods when investigating the short-range order and elastic properties of two equimolar WCrTaTi and WVTaTi W-HEAs, and two WCrTi and WCrY W-SAs. We found that structures after MC-DFT calculation have lower cohesive energies than SQS structures, with shorter lattice constants, and large elastic properties values. Furthermore, distinct element segregation was studied by calculating the SRO parameter and radius distribution function. The total density of states suggested that the existence of SRO could improve the stability of the structure.

==> 4_Discussion.tex <==
\section{Discussion} \label{sec_Discussion}


\subsection{structure properties of tungsten-based PFMs}

Section~\ref{MC-DFT-results} presented the energy evaluation of the tungsten-based PFMs with 1000 MC swaps from the gradient decreasing temperature 800K, 500k, and 100K. The main objective was to determine the most energy-stable structures in the presence of SRO.
%
First, the results indicate that the presence of SRO can significantly reduce the system energy by 4-9eV(0.03 eV $\sim$ 0.07 eV/atom). Analysis of the SRO figures revealed that the reduction in energy originates from various factors. For instance, in HEA1, the SRO values of Ta-Ta, Cr-Cr are positive in the first shell and negative in the second shell, and Ta-Cr is the opposite case. This indicates a Ta-Cr sublattice bcc structure, where Ta(Cr) atom is at the body center position, and Cr(Ta) atom is at the corner position. Additionally, Ti-Ti clusters and repulsion of W-Ti were observed. For HEA2, a similar phenomenon was observed with bcc sublattice structure for Ta-V, and more W-Ti pair and fewer W-W and Ti-Ti pairs were detected.
In SA1 and SA2, The appearance of the cubic Cr sublattice was detected, as the average SRO values of W-Cr and Cr-Cr are zero with opposite SRO values in the first and second shells. This observation is consistent with the findings of Kang\cite{kangdensity} in MC-DFT simulation of FeMnCoCrNi alloys, who confirm the arrangement of Cr atoms is the precursor of $L1_{2}$ phase, and it will transfer into $L1_{2}$ phase with higher concentrations of Cr. The results obtained from this study provide valuable insights into the effects of SRO on the energy evaluation of W-based PFMs









%In this Section we consider the most important implications of our results. % disloUCLA


